First investigation of a novel 2D position-sensitive semiconductor detector concept

This paper presents a first study of the performance of a novel 2D position-sensitive microstrip detector, where the resistive charge division method was implemented by replacing the metallic electrodes with resistive electrodes made of polycrystalline silicon. A characterization of two proof-of-concept prototypes with different values of the electrode resistivity was carried out using a pulsed Near Infra-Red laser. The experimental data were compared with the electrical simulation of the sensor equivalent circuit coupled to simple electronics readout circuits. The good agreement between experimental and simulation results establishes the soundness of resistive charge division method in silicon microstrip sensors and validates the developed simulation as a tool for the optimization of future sensor prototypes. Spatial resolution in the strip length direction depends on the ionizing event position. The average value obtained from the protype analysis is close to 1.2% of the strip length for a 6 MIP signal.

==> 0410217.tex <==
%auto-ignore
